Classical simulation and model concentration in passive linear optics

Passive linear optics is a restricted model of quantum computation, with complexity-theoretic evidence of quantum advantage for sampling tasks and low losses that make it attractive for near-term algorithms. In qubit architectures, a body of work has revealed a close connection between barren plateaus and classical simulability. Whether an analogous tradeoff exists for bosonic systems remains largely unexplored. Building on a recently developed representation-theoretic framework for moments of random passive linear-optical circuits, we characterize the concentration of expectation values for relevant families of particle-number-preserving observables by evaluating their projections into irreducible representations of the unitary group and analyzing their asymptotic scaling. We show that concentration is governed by the misalignment of the projections into irreducible representations of the input state and the observable, giving a unified representation-theoretic interpretation of generalized entanglement and locality in the bosonic setting. We further relate these concentration properties to existing classical simulation techniques, identifying broad classes of trainable observables that admit efficient classical simulation. Conversely, we identify Fock-state inputs and observables that appear to evade exponential concentration while retaining a polynomially large signal component not accessible to known efficient classical simulation methods. The separation is only partial: most of the signal remains classically tractable, and the residual part, while not exponentially suppressed, is small enough that a truncation serves as a classical surrogate with polynomially small error. Our framework nonetheless provides a systematic route for searching for regimes that unambiguously combine the absence of exponential concentration and lies beyond known efficient classical simulation methods.

==> plots/Concentration_Comparison_legend.tex <==
% triple_variance_legend — standalone legend box for triple_variance_plot.tex
% Requires only: \usepackage{tikz}  (xcolor 'gray' is standard)
% One entry per colour (observable); the two grey entries encode the
% min/max bunching line style (solid = max, densely dotted = min).
% Layout is a 4-column x 2-row grid; change \lcolI..\lcolIV or row spacing to reshape.
  \definecolor{smpcol}{rgb}{0.0824,0.3961,0.7529}
  \definecolor{dmpcol}{rgb}{0.3922,0.7098,0.9647}
  \definecolor{singleirrepcol}{rgb}{0.1804,0.4902,0.1961}
  \definecolor{polyparitycol}{rgb}{0.4157,0.1059,0.6039}
  \definecolor{paritysumcol}{rgb}{0.7765,0.1569,0.1569}
  \definecolor{projectorcol}{rgb}{0.9020,0.3176,0.0000}
\begin{tikzpicture}
  % --- column x-origins and row y-positions (cm) ---
  \def\lcolI{0}\def\lcolII{3.7}\def\lcolIII{7.4}\def\lcolIV{11.1}
  \def\lrowI{0}\def\lrowII{-0.6}
  % --- coloured line entry (no marker, matching the plot) ---
  \newcommand{\legcolor}[4]{% #1=x #2=y #3=color #4=label
    \draw[#3, line width=1.5pt] (#1,#2) -- ++(0.6,0);
    \node[anchor=west, inner sep=1pt, font=\footnotesize] at (#1+0.75,#2) {#4};}
  % --- grey line-style entry (line grey, text black) ---
  \newcommand{\legstyle}[4]{% #1=x #2=y #3=solid/densely dotted #4=label
    \draw[gray, line width=1.5pt, #3] (#1,#2) -- ++(0.6,0);
    \node[anchor=west, inner sep=1pt, font=\footnotesize] at (#1+0.75,#2) {#4};}
  \begin{scope}[local bounding box=leg]
    % row 1 (observables)
    \legcolor{\lcolI}{\lrowI}{smpcol}{$\hat{n}_0^p$}
    \legcolor{\lcolII}{\lrowI}{dmpcol}{$\hat{n}_{i_1} \dots \hat{n}_{i_p}$}
    \legcolor{\lcolIII}{\lrowI}{singleirrepcol}{$\prod_{k=1}^p \frac{\hat{a}^\dagger_{i_k} \hat{a}_{j_k} + \hat{a}^\dagger_{j_k} \hat{a}_{i_k}}{\sqrt{2}}$}
    \legcolor{\lcolIV}{\lrowI}{polyparitycol}{$\prod_{i=1}^p (-1)^{\alpha_i \hat{n}_{i}^2}$}
    % row 2 (observables + grey style key)
    \legcolor{\lcolI}{\lrowII}{paritysumcol}{$\prod_{i=1}^p (-1)^{\hat{n}_{i}}$}
    \legcolor{\lcolII}{\lrowII}{projectorcol}{$\ketbra{S}{S}$}
    \legstyle{\lcolIII}{\lrowII}{solid}{$\ket{n, 0, \dots, 0}$}
    \legstyle{\lcolIV}{\lrowII}{densely dotted}{$\ket{1, \dots, 1, 0, \dots,0}$}
  \end{scope}
  % surrounding rectangle with a little padding (reduced vertical padding => shorter box)
  \draw[black]
    ([xshift=-6pt,yshift=-2pt]leg.south west)
    rectangle
    ([xshift=6pt,yshift=2pt]leg.north east);
\end{tikzpicture}

==> plots/Fock_States/Fock_States_Kstar_Scatter.tex <==
% Fock_States_Kstar_Scatter — generated by Projector_Fock_States.ipynb
% Requires: \usepackage{pgfplots} \pgfplotsset{compat=1.18}

\begin{tikzpicture}
  \definecolor{tabred60}{rgb}{0.9035,0.4918,0.4941}
  \definecolor{tabblue60}{rgb}{0.4729,0.6800,0.8235}
  \definecolor{barbot10k7}{rgb}{0.4729,0.6800,0.8235}
  \definecolor{bartop10k7}{rgb}{0.4729,0.6800,0.8235}
  \definecolor{barbot10k8}{rgb}{0.5135,0.6623,0.7925}
  \definecolor{bartop10k8}{rgb}{0.5135,0.6623,0.7925}
  \definecolor{barbot10k9}{rgb}{0.6317,0.6106,0.7021}
  \definecolor{bartop10k9}{rgb}{0.5472,0.6475,0.7667}
  \definecolor{barbot10k10}{rgb}{0.7684,0.5508,0.5975}
  \definecolor{bartop10k10}{rgb}{0.5928,0.6276,0.7318}
  \definecolor{barbot20k15}{rgb}{0.4932,0.6711,0.8080}
  \definecolor{bartop20k15}{rgb}{0.4729,0.6800,0.8235}
  \definecolor{barbot20k16}{rgb}{0.5354,0.6527,0.7757}
  \definecolor{bartop20k16}{rgb}{0.5135,0.6623,0.7925}
  \definecolor{barbot20k17}{rgb}{0.5759,0.6350,0.7447}
  \definecolor{bartop20k17}{rgb}{0.5320,0.6542,0.7783}
  \definecolor{barbot20k18}{rgb}{0.6182,0.6165,0.7124}
  \definecolor{bartop20k18}{rgb}{0.5624,0.6409,0.7551}
  \definecolor{barbot20k19}{rgb}{0.6975,0.5818,0.6517}
  \definecolor{bartop20k19}{rgb}{0.5759,0.6350,0.7447}
  \definecolor{barbot20k20}{rgb}{0.8073,0.5338,0.5678}
  \definecolor{bartop20k20}{rgb}{0.5928,0.6276,0.7318}
  \definecolor{barbot30k22}{rgb}{0.4729,0.6800,0.8235}
  \definecolor{bartop30k22}{rgb}{0.4729,0.6800,0.8235}
  \definecolor{barbot30k23}{rgb}{0.5000,0.6682,0.8029}
  \definecolor{bartop30k23}{rgb}{0.4864,0.6741,0.8132}
  \definecolor{barbot30k24}{rgb}{0.5287,0.6556,0.7809}
  \definecolor{bartop30k24}{rgb}{0.5135,0.6623,0.7925}
  \definecolor{barbot30k25}{rgb}{0.5574,0.6431,0.7589}
  \definecolor{bartop30k25}{rgb}{0.5253,0.6571,0.7835}
  \definecolor{barbot30k26}{rgb}{0.5979,0.6254,0.7279}
  \definecolor{bartop30k26}{rgb}{0.5472,0.6475,0.7667}
  \definecolor{barbot30k27}{rgb}{0.6266,0.6128,0.7060}
  \definecolor{bartop30k27}{rgb}{0.5574,0.6431,0.7589}
  \definecolor{barbot30k28}{rgb}{0.6671,0.5951,0.6750}
  \definecolor{bartop30k28}{rgb}{0.5675,0.6387,0.7512}
  \definecolor{barbot30k29}{rgb}{0.7347,0.5656,0.6233}
  \definecolor{bartop30k29}{rgb}{0.5827,0.6320,0.7396}
  \definecolor{barbot30k30}{rgb}{0.8259,0.5257,0.5535}
  \definecolor{bartop30k30}{rgb}{0.5928,0.6276,0.7318}

  \begin{axis}[
    ylabel={$(\arg \displaystyle\max_{k \leq n} \|P_k(\ket{R}\bra{R})\|_2^2)/n$},
    ymin=0, ymax=1.06,
    xmin=0.5, xmax=3.5,
    xtick={1,2,3},
    xticklabels={$n=10$,$n=20$,$n=30$},
    ymajorgrids=true, grid style={dashed, gray!40},
    colormap={mymap}{color(0pt)=(tabred60);color(1pt)=(tabblue60)},
    colorbar,
    colorbar style={ylabel={$\|R\|_2/n$}, font=\small},
    point meta min=0, point meta max=1,
    tick label style={font=\small},
    label style={font=\small},
    title style={font=\small},
    width=0.80\linewidth, height=0.60\linewidth,
  ]
  \fill[bottom color=barbot10k7, top color=bartop10k7]
    (axis cs:0.6750,0) -- (axis cs:0.8375,0) --
    (axis cs:0.8375,0.700000) -- (axis cs:0.6750,0.700000) -- cycle;
  \fill[bottom color=barbot10k8, top color=bartop10k8]
    (axis cs:0.8375,0) -- (axis cs:1.0000,0) --
    (axis cs:1.0000,0.800000) -- (axis cs:0.8375,0.800000) -- cycle;
  \fill[bottom color=barbot10k9, top color=bartop10k9]
    (axis cs:1.0000,0) -- (axis cs:1.1625,0) --
    (axis cs:1.1625,0.900000) -- (axis cs:1.0000,0.900000) -- cycle;
  \fill[bottom color=barbot10k10, top color=bartop10k10]
    (axis cs:1.1625,0) -- (axis cs:1.3250,0) --
    (axis cs:1.3250,1.000000) -- (axis cs:1.1625,1.000000) -- cycle;
  \fill[bottom color=barbot20k15, top color=bartop20k15]
    (axis cs:1.6750,0) -- (axis cs:1.7833,0) --
    (axis cs:1.7833,0.750000) -- (axis cs:1.6750,0.750000) -- cycle;
  \fill[bottom color=barbot20k16, top color=bartop20k16]
    (axis cs:1.7833,0) -- (axis cs:1.8917,0) --
    (axis cs:1.8917,0.800000) -- (axis cs:1.7833,0.800000) -- cycle;
  \fill[bottom color=barbot20k17, top color=bartop20k17]
    (axis cs:1.8917,0) -- (axis cs:2.0000,0) --
    (axis cs:2.0000,0.850000) -- (axis cs:1.8917,0.850000) -- cycle;
  \fill[bottom color=barbot20k18, top color=bartop20k18]
    (axis cs:2.0000,0) -- (axis cs:2.1083,0) --
    (axis cs:2.1083,0.900000) -- (axis cs:2.0000,0.900000) -- cycle;
  \fill[bottom color=barbot20k19, top color=bartop20k19]
    (axis cs:2.1083,0) -- (axis cs:2.2167,0) --
    (axis cs:2.2167,0.950000) -- (axis cs:2.1083,0.950000) -- cycle;
  \fill[bottom color=barbot20k20, top color=bartop20k20]
    (axis cs:2.2167,0) -- (axis cs:2.3250,0) --
    (axis cs:2.3250,1.000000) -- (axis cs:2.2167,1.000000) -- cycle;
  \fill[bottom color=barbot30k22, top color=bartop30k22]
    (axis cs:2.6750,0) -- (axis cs:2.7472,0) --
    (axis cs:2.7472,0.733333) -- (axis cs:2.6750,0.733333) -- cycle;
  \fill[bottom color=barbot30k23, top color=bartop30k23]
    (axis cs:2.7472,0) -- (axis cs:2.8194,0) --
    (axis cs:2.8194,0.766667) -- (axis cs:2.7472,0.766667) -- cycle;
  \fill[bottom color=barbot30k24, top color=bartop30k24]
    (axis cs:2.8194,0) -- (axis cs:2.8917,0) --
    (axis cs:2.8917,0.800000) -- (axis cs:2.8194,0.800000) -- cycle;
  \fill[bottom color=barbot30k25, top color=bartop30k25]
    (axis cs:2.8917,0) -- (axis cs:2.9639,0) --
    (axis cs:2.9639,0.833333) -- (axis cs:2.8917,0.833333) -- cycle;
  \fill[bottom color=barbot30k26, top color=bartop30k26]
    (axis cs:2.9639,0) -- (axis cs:3.0361,0) --
    (axis cs:3.0361,0.866667) -- (axis cs:2.9639,0.866667) -- cycle;
  \fill[bottom color=barbot30k27, top color=bartop30k27]
    (axis cs:3.0361,0) -- (axis cs:3.1083,0) --
    (axis cs:3.1083,0.900000) -- (axis cs:3.0361,0.900000) -- cycle;
  \fill[bottom color=barbot30k28, top color=bartop30k28]
    (axis cs:3.1083,0) -- (axis cs:3.1806,0) --
    (axis cs:3.1806,0.933333) -- (axis cs:3.1083,0.933333) -- cycle;
  \fill[bottom color=barbot30k29, top color=bartop30k29]
    (axis cs:3.1806,0) -- (axis cs:3.2528,0) --
    (axis cs:3.2528,0.966667) -- (axis cs:3.1806,0.966667) -- cycle;
  \fill[bottom color=barbot30k30, top color=bartop30k30]
    (axis cs:3.2528,0) -- (axis cs:3.3250,0) --
    (axis cs:3.3250,1.000000) -- (axis cs:3.2528,1.000000) -- cycle;
  \addplot[scatter, only marks, scatter src=explicit, mark=*, mark size=2pt, forget plot]
    coordinates {(8,0.0034720608)[1.0] (16,1.31e-05)[0.7] (32,1.46e-14)[0.4]};
  \end{axis}
\end{tikzpicture}


==> plots/Parity_Operators/Sum_Poly_Parity_Operators_Purities.tex <==
% Combined purity evolution: sum-parity vs poly-parity observables
% Requires: \usepackage{pgfplots} \pgfplotsset{compat=1.18} \usepgfplotslibrary{groupplots}

\begin{tikzpicture}
  \definecolor{col0}{rgb}{0.1216,0.4667,0.7059}
  \definecolor{col1}{rgb}{1.0000,0.4980,0.0549}
  \definecolor{col2}{rgb}{0.1725,0.6275,0.1725}
  \definecolor{col3}{rgb}{0.8392,0.1529,0.1569}
  \definecolor{col4}{rgb}{0.5804,0.4039,0.7412}
  \begin{groupplot}[
    group style={
      group size=2 by 1,
      horizontal sep=1.6cm,
      ylabels at=edge left,
    },
    ymode=log,
    xlabel={Irrep $k$},
    tick label style={font=\small},
    label style={font=\small},
    title style={font=\small},
    legend style={font=\small},
    width=0.48\linewidth,
    height=0.48\linewidth,
  ]

  % --- Panel 1: sum-parity observable ---
  \nextgroupplot[
    ylabel={$\|P_{k}(O)\|_2^2/\|O\|_\infty^2$},
    title={$O=\displaystyle\prod_{i=1}^{\log_2 n}(-1)^{\hat n_i}$},
    legend to name=combinedlegend,
    legend columns=5,
  ]
    \addplot[col0, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,1.6) (1,2.0) (2,6.4)};
    \addlegendentry{$n=2$}
    \addplot[col1, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,10.193939393939393) (1,27.927272727272726) (2,56.287179487179486) (3,74.47272727272727) (4,161.11888111888112)};
    \addlegendentry{$n=4$}
    \addplot[col2, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,3980.862059822889) (1,13446.875112682894) (2,28730.727427729984) (3,48443.33569100617) (4,69267.47559808612) (5,86007.90513833992) (6,93295.68117759303) (7,83668.49011857707) (8,63472.64767616192)};
    \addlegendentry{$n=8$}
    \addplot[col3, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,3510106289.860451) (1,13487673755.701231) (2,31548567475.501892) (3,57434405486.095436) (4,88871019899.2191) (5,121877767426.64168) (6,151491793799.02136) (7,172774404605.54953) (8,181889605981.70905) (9,177007678691.84454) (10,158803591361.81738) (11,130395197928.02562) (12,96691108371.58745) (13,63267952926.113304) (14,35044981529.30299) (15,15099176390.551298) (16,4037577179.4576707)};
    \addlegendentry{$n=16$}
    \addplot[col4, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,1.3336285591120915e+22) (1,5.78460052865191e+22) (2,1.4858576929156846e+23) (3,2.9287824269849873e+23) (4,4.87995703262304e+23) (5,7.213489623323249e+23) (6,9.726934843661461e+23) (7,1.217632769564853e+24) (8,1.4316099420062367e+24) (9,1.5936265675043018e+24) (10,1.6890874445655574e+24) (11,1.7114017688412476e+24) (12,1.6622284947265898e+24) (13,1.5504922575730676e+24) (14,1.3904797655465099e+24) (15,1.1994325169448223e+24) (16,9.950732010441713e+23) (17,7.934484837987568e+23) (18,6.073603137041665e+23) (19,4.455186783636328e+23) (20,3.124095006328677e+23) (21,2.0875668039537555e+23) (22,1.3238372750834582e+23) (23,7.925445586559782e+22) (24,4.449029171808729e+22) (25,2.32124456779036e+22) (26,1.1124563956756543e+22) (27,4.819002724234621e+21) (28,1.8440430836987873e+21) (29,6.020931162821485e+20) (30,1.5842953539519323e+20) (31,3.0142561119813165e+19) (32,3.1482230502915973e+18)};
    \addlegendentry{$n=32$}

  % --- Panel 2: poly-parity observable ---
  \nextgroupplot[
    %ylabel={$\|P_{k}(G_p)\|_2^2/\|G_p\|_\infty^2$},
    title={$O = \displaystyle\prod_{i=1}^{\log_2 n} (-1)^{\alpha_i \hat n^2_i}$},
  ]
    \addplot[col0, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,5.8) (1,1.0) (2,3.2)};
    \addplot[col1, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,98.06463465578749) (1,72.93213197424326) (2,43.34487935252396) (3,56.51953407559629) (4,59.138819941849)};
    \addplot[col2, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,96927.55717270932) (1,93129.68479771548) (2,56275.354478091336) (3,60029.31207206687) (4,54704.233298792344) (5,50014.85231249668) (6,40980.4618345982) (7,26288.603735814704) (8,11963.940297715064)};
    \addplot[col3, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,222129394251.31448) (1,239746710618.55933) (2,161727706255.2208) (3,147311879735.72504) (4,143279979195.77982) (5,126456851510.201) (6,111435502399.28632) (7,98169191544.46954) (8,82373780595.3728) (9,64011344858.98318) (10,45540313260.8401) (11,29431138767.66445) (12,17211999367.416798) (13,8949803179.346315) (14,3910035293.7109413) (15,1292719231.6221707) (16,254259032.48693094)};
    \addplot[col4, solid, mark=*, line width=1.5pt, mark size=2pt]
      coordinates {(0,2.4366753629482546e+24) (1,2.798401866349462e+24) (2,2.0269357282368975e+24) (3,1.7443660159138663e+24) (4,1.688278091437802e+24) (5,1.528405766964867e+24) (6,1.3385175854870296e+24) (7,1.1825852492660668e+24) (8,1.0471595362028269e+24) (9,9.111539969124358e+23) (10,7.663660804324106e+23) (11,6.198797232977872e+23) (12,4.84269559061769e+23) (13,3.676575310537958e+23) (14,2.7243065199126206e+23) (15,1.972944842893621e+23) (16,1.3927913409516593e+23) (17,9.531840681026644e+22) (18,6.288878344776823e+22) (19,3.98488485264849e+22) (20,2.4188414317228827e+22) (21,1.4026896370979425e+22) (22,7.739500200162697e+21) (23,4.039546989905327e+21) (24,1.9788929670414504e+21) (25,9.004809115492203e+20) (26,3.754154545604615e+20) (27,1.4082614316239808e+20) (28,4.6403813736890245e+19) (29,1.2977639004681992e+19) (30,2.912352328380069e+18) (31,4.7062701858143334e+17) (32,4.149885174223177e+16)};

  \end{groupplot}

  % shared legend below both panels
  \node at ($(group c1r1.south)!0.5!(group c2r1.south)$) [yshift=-1.3cm] {\pgfplotslegendfromname{combinedlegend}};

\end{tikzpicture}

==> plots/Product_Photon_Number/First_Moment_Product_Number_Operators.tex <==
% sec_first_moment — generated by Product_Number_Operator.ipynb
% Requires: \usepackage{pgfplots} \pgfplotsset{compat=1.18}

% --- p=2 ---
\begin{tikzpicture}
  \definecolor{smpcol}{rgb}{0.0824,0.3961,0.7529}
  \definecolor{dmpcol}{rgb}{0.7765,0.1569,0.1569}
  \begin{axis}[
    ymode=log,
    xlabel={$n$},
    ylabel={$\mathbb{E}[f_U]$},
    title={$p=2$},
    legend pos=north east,
    title style={font=\huge},
    xlabel style={font=\huge},
    ylabel style={font=\huge},
    legend style={font=\huge, inner sep=8pt},
    tick label style={font=\huge},
    label style={font=\huge},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    \addplot[smpcol, solid, mark=*, line width=1.5pt, mark size=3pt] coordinates {(2,0.175) (3,0.0873015873015873) (4,0.052083333333333336) (5,0.034545454545454546) (6,0.024572649572649572) (7,0.018367346938775512) (8,0.014246323529411764) (9,0.011371020142949967) (10,0.009285714285714286) (11,0.007725476104922745) (12,0.006527777777777778) (13,0.005588428665351742) (14,0.00483814215341309) (15,0.004229390681003585) (16,0.003728693181818182) (17,0.003311913000494315) (18,0.0029612946279612947) (19,0.0026635414447048794) (20,0.0024085365853658536) (21,0.002188472288140062) (22,0.001997245179063361) (23,0.0018300285564895628) (24,0.0016829648526077098) (25,0.0015529411764705883) (26,0.0014374232443898627) (27,0.0013343309639605935) (28,0.0012419441460794845) (29,0.001158830286785304) (30,0.0010837887067395265) (31,0.0010158069471284871) (32,0.0009540264423076923) (33,0.0008977152803475734) (34,0.0008462464269595306) (35,0.000799080195458465)};
    \addlegendentry{$\hat n_1^p$}
    \addplot[dmpcol, solid, mark=square*, line width=1.5pt, mark size=3pt] coordinates {(2,0.1) (3,0.07142857142857142) (4,0.041666666666666664) (5,0.030303030303030304) (6,0.021367521367521368) (7,0.016666666666666666) (8,0.012867647058823529) (9,0.010526315789473684) (10,0.008571428571428572) (11,0.007246376811594203) (12,0.006111111111111111) (13,0.005291005291005291) (14,0.004574243490499648) (15,0.004032258064516129) (16,0.0035511363636363635) (17,0.0031746031746031746) (18,0.0028361695028361693) (19,0.002564102564102564) (20,0.002317073170731707) (21,0.0021141649048625794) (22,0.0019283746556473828) (23,0.0017730496453900707) (24,0.0016298185941043086) (25,0.0015082956259426853) (26,0.0013955565479513228) (27,0.0012987012987012987) (28,0.0012083780880773364) (29,0.0011299435028248586) (30,0.001056466302367942) (31,0.0009920634920634924) (32,0.0009314903846153845) (33,0.000877963125548727) (34,0.0008274409508048743) (35,0.0007824726134585289)};
    \addlegendentry{$\prod_{i=1}^p \hat n_i$}
  \end{axis}
\end{tikzpicture}

% --- p=log2n ---
\begin{tikzpicture}
  \definecolor{smpcol}{rgb}{0.0824,0.3961,0.7529}
  \definecolor{dmpcol}{rgb}{0.7765,0.1569,0.1569}
  \begin{axis}[
    ymode=log,
    xlabel={$n$},
    title={$p=\lfloor\log_2 n \rfloor$},
    legend pos=north east,
    title style={font=\huge},
    xlabel style={font=\huge},
    ylabel style={font=\huge},
    legend style={font=\huge, inner sep=8pt},
    tick label style={font=\huge},
    label style={font=\huge},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    \addplot[smpcol, solid, mark=*,line width=1.5pt, mark size=3pt] coordinates {(2,0.25) (3,0.16666666666666666) (4,0.052083333333333336) (5,0.034545454545454546) (6,0.024572649572649572) (7,0.018367346938775512) (8,0.004193474264705882) (9,0.0030250523427911343) (10,0.002253246753246753) (11,0.0017231241629373142) (12,0.0013470441595441595) (13,0.0010728916054359842) (14,0.0008683522670151804) (15,0.0007126642771804062) (16,0.00012031595974682486) (17,9.570570627071388e-05) (18,7.70777316694579e-05) (19,6.276895182170543e-05) (20,5.1631502714528806e-05) (21,4.2858146232386296e-05) (22,3.587150126462795e-05) (23,3.0252198466717244e-05) (24,2.569133845667897e-05) (25,2.1958453000939127e-05) (26,1.8879550412687365e-05) (27,1.632183878685669e-05) (28,1.4182944672073574e-05) (29,1.2383204288721539e-05) (30,1.0860084480743743e-05) (31,9.564099268069183e-06) (32,1.1173058578759706e-06) (33,9.635148404423467e-07) (34,8.344389439166666e-07) (35,7.255663320700857e-07)};
    \addlegendentry{$\hat n_1^p$}
    \addplot[dmpcol, solid, mark=square*, line width=1.5pt, mark size=3pt] coordinates {(2,0.25) (3,0.16666666666666666) (4,0.041666666666666664) (5,0.030303030303030304) (6,0.021367521367521368) (7,0.016666666666666666) (8,0.003812636165577342) (9,0.0027290448343079924) (10,0.0021645021645021645) (11,0.0016983695652173913) (12,0.0013221153846153847) (13,0.0010912698412698413) (14,0.000896551724137931) (15,0.0007338709677419355) (16,0.00013577874331550802) (17,0.00011261261261261261) (18,9.300798774482986e-05) (19,7.654784240150094e-05) (20,6.28150068876104e-05) (21,5.355884425651868e-05) (22,4.556823243224723e-05) (23,3.869751210176745e-05) (24,3.2809420064322116e-05) (25,2.857133822727619e-05) (26,2.4849530689602437e-05) (27,2.1588559259266532e-05) (28,1.8737002045593702e-05) (29,1.6586239941933896e-05) (30,1.4670728153768044e-05) (31,1.2967176053113507e-05) (32,1.8252322905526788e-06) (33,1.5880839703832216e-06) (34,1.3804970557781935e-06) (35,1.1990544586655765e-06)};
    \addlegendentry{$\prod_{i=1}^p \hat n_i$}
  \end{axis}
\end{tikzpicture}

% --- p=sqrtn ---
\begin{tikzpicture}
  \definecolor{smpcol}{rgb}{0.0824,0.3961,0.7529}
  \definecolor{dmpcol}{rgb}{0.7765,0.1569,0.1569}
  \begin{axis}[
    ymode=log,
    xlabel={$n$},
    title={$p=\lfloor\sqrt n \rfloor$},
    legend pos=north east,
    title style={font=\huge},
    xlabel style={font=\huge},
    ylabel style={font=\huge},
    legend style={font=\huge, inner sep=7pt},
    tick label style={font=\huge},
    label style={font=\huge},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    \addplot[smpcol, solid, mark=*,line width=1.5pt, mark size=3pt] coordinates {(2,0.25) (3,0.16666666666666666) (4,0.052083333333333336) (5,0.034545454545454546) (6,0.024572649572649572) (7,0.018367346938775512) (8,0.014246323529411764) (9,0.0030250523427911343) (10,0.002253246753246753) (11,0.0017231241629373142) (12,0.0013470441595441595) (13,0.0010728916054359842) (14,0.0008683522670151804) (15,0.0007126642771804062) (16,0.00012031595974682486) (17,9.570570627071388e-05) (18,7.70777316694579e-05) (19,6.276895182170543e-05) (20,5.1631502714528806e-05) (21,4.2858146232386296e-05) (22,3.587150126462795e-05) (23,3.0252198466717244e-05) (24,2.569133845667897e-05) (25,3.640693155752867e-06) (26,3.0203173793390827e-06) (27,2.5225664976951613e-06) (28,2.1200746587788773e-06) (29,1.792237579122913e-06) (30,1.5233899802617118e-06) (31,1.3015128371238653e-06) (32,1.1173058578759706e-06) (33,9.635148404423467e-07) (34,8.344389439166666e-07) (35,7.255663320700857e-07)};
    \addlegendentry{$\hat n_1^p$}
    \addplot[dmpcol, solid, mark=square*, line width=1.5pt, mark size=3pt] coordinates {(2,0.25) (3,0.16666666666666666) (4,0.041666666666666664) (5,0.030303030303030304) (6,0.021367521367521368) (7,0.016666666666666666) (8,0.012867647058823529) (9,0.0027290448343079924) (10,0.0021645021645021645) (11,0.0016983695652173913) (12,0.0013221153846153847) (13,0.0010912698412698413) (14,0.000896551724137931) (15,0.0007338709677419355) (16,0.00013577874331550802) (17,0.00011261261261261261) (18,9.300798774482986e-05) (19,7.654784240150094e-05) (20,6.28150068876104e-05) (21,5.355884425651868e-05) (22,4.556823243224723e-05) (23,3.869751210176745e-05) (24,3.2809420064322116e-05) (25,5.375983000844273e-06) (26,4.592193271438524e-06) (27,3.9152217010655265e-06) (28,3.332410511960698e-06) (29,2.832079002430761e-06) (30,2.4036146692258346e-06) (31,2.0957052207051507e-06) (32,1.8252322905526788e-06) (33,1.5880839703832216e-06) (34,1.3804970557781935e-06) (35,1.1990544586655765e-06)};
    \addlegendentry{$\prod_{i=1}^p \hat n_i$}
  \end{axis}
\end{tikzpicture}



==> plots/Product_Photon_Number/Product_Number_Operators_Purities.tex <==
% sec1_product_comparison — generated by Product_Number_Operator.ipynb
% Include with: \input{sec1_product_comparison.tex}
% Requires: \usepackage{pgfplots} \pgfplotsset{compat=1.18}
\begin{tikzpicture}
  \definecolor{col0}{rgb}{0.1216,0.4667,0.7059}
  \definecolor{col1}{rgb}{1.0000,0.4980,0.0549}
  \definecolor{col2}{rgb}{0.1725,0.6275,0.1725}
  \definecolor{col3}{rgb}{0.8392,0.1529,0.1569}
  \definecolor{col4}{rgb}{0.5804,0.4039,0.7412}
  \begin{axis}[
    ymode=log,
    xlabel={Irrep $k$},
    ylabel={$\|P_k(O)\|_2^2 / \|O\|_\infty^2$},
    legend pos=outer north east,
    legend style={font=\small},
    tick label style={font=\small},
    label style={font=\small},
    title style={font=\small},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    % --- Custom legend entries ---
    \addlegendimage{col0, line width=1.5pt}
    \addlegendentry{$n=2$}
    \addlegendimage{col1, line width=1.5pt}
    \addlegendentry{$n=4$}
    \addlegendimage{col2, line width=1.5pt}
    \addlegendentry{$n=8$}
    \addlegendimage{col3, line width=1.5pt}
    \addlegendentry{$n=16$}
    \addlegendimage{col4, line width=1.5pt}
    \addlegendentry{$n=32$}
    \addlegendimage{gray, dotted, mark=o, line width=1.5pt, mark size=3pt}
    \addlegendentry{$\hat{n}_1^{\log_2(n)}$}
    \addlegendimage{gray, solid, mark=*, line width=1.5pt, mark size=3pt}
    \addlegendentry{$\prod_{i=1}^{\log_2 n}\hat{n}_i$}
    % --- Data plots (excluded from legend) ---
    \addplot[col0, dotted, mark=o, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,0.625) (1,1.125)};
    \addplot[col0, solid, mark=*, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,0.625) (1,1.125)};
    \addplot[col1, dotted, mark=o, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,0.8951822916666666) (1,3.639453125) (2,0.7583333333333333)};
    \addplot[col1, solid, mark=*, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,0.5729166666666666) (1,1.85625) (2,4.008333333333334)};
    \addplot[col2, dotted, mark=o, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,8.622282701380113) (1,76.8034879784835) (2,68.86176614200367) (3,5.388408460115132)};
    \addplot[col2, solid, mark=*, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,7.1272996853062205) (1,39.26924951267057) (2,117.68082788671025) (3,175.5985488412389)};
    \addplot[col3, dotted, mark=o, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,21760.690278268277) (1,366066.5965935669) (2,796040.9993659487) (3,299214.2394919938) (4,13376.247414101239)};
    \addplot[col3, solid, mark=*, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,27713.396656342367) (1,237103.5047264847) (2,962836.4115169662) (3,2147191.7295587026) (4,2186955.5613470464)};
    \addplot[col4, dotted, mark=o, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,24719227705910.777) (1,686709936091008.5) (2,2836120661348268.5) (3,2668130901670963.0) (4,562964246032293.2) (5,16926632352767.074)};
    \addplot[col4, solid, mark=*, line width=1.5pt, mark size=3pt, forget plot]
      coordinates {(0,65967045478943.73) (1,797049840616727.1) (2,4313780607054207.0) (3,1.2995817294272024e+16) (4,2.1692738215542628e+16) (5,1.599157169572476e+16)};
  \end{axis}
\end{tikzpicture}

==> plots/Product_Photon_Number/sec3_observable_only.tex <==
% sec3_observable_only — generated by Product_Number_Operator.ipynb
% Requires: \usepackage{pgfplots} \pgfplotsset{compat=1.18}


% ---- log2n ----
\begin{tikzpicture}
  \definecolor{smpcol}{rgb}{0.0824,0.3961,0.7529}
  \definecolor{dmpcol}{rgb}{0.7765,0.1569,0.1569}
  \begin{axis}[
    ymode=log,
    xlabel={$n$},
    ylabel={$\displaystyle\sum_{k\geq k_0}\frac{\|P_k(O)\|_2^2}{\|O\|_\infty^2\, d_k^{(n)}}$},
    title={$p = \lfloor\log_2 n\rfloor$},
    legend pos=outer north east,
    legend style={font=\large},
    tick label style={font=\large},
    label style={font=\large},
    title style={font=\large},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    \addplot[smpcol, solid, mark=*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.7) (3,1.6507936507936507) (4,0.9535669191919192) (5,2.4980960372960372) (6,7.724225568670013) (7,26.827811941102972) (8,8.927256490107608) (9,29.422446907282467) (10,104.16023171959797) (11,390.9679167283678) (12,1540.8550315326004) (13,6328.589575899145) (14,26928.848605752093) (15,118153.73876163572) (16,22121.40099611427) (17,91540.80993217549) (18,389053.4355269806) (19,1693538.7089469354) (20,7532670.074926362) (21,34165792.34784907) (22,157747283.66789332) (23,740282063.3614491) (24,3526277312.5205913) (25,17029717957.892193) (26,83294529325.28702) (27,412230063258.4772) (28,2062604383711.5325) (29,10426083475046.992) (30,53206343860639.22) (31,273954566965477.03) (32,24887579877252.156) (33,122985716518034.9) (34,613248553322498.5) (35,3083959473927130.5)};
    \addplot[smpcol, solid, mark=square*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.075) (3,0.09523809523809523) (4,0.000615530303030303) (5,0.0008354312354312355) (6,0.0014606792384570162) (7,0.00307224930788642) (8,8.323666059248535e-06) (9,1.5938077230151574e-05) (10,3.420971654432524e-05) (11,8.078660269041226e-05) (12,0.00020686725430599153) (13,0.0005678229230054961) (14,0.001655357625712395) (15,0.005086997888380507) (16,4.943616865457458e-06) (17,1.368104080635521e-05) (18,3.962228106770109e-05) (19,0.00011956513221986061) (20,0.00037451766451742155) (21,0.001213711514007376) (22,0.0040577573154919975) (23,0.013960046851328506) (24,0.04931150628547201) (25,0.1784881181207702) (26,0.6608489169520245) (27,2.4988448392865714) (28,9.63612693257353) (29,37.84723707995414) (30,151.22704814010194) (31,614.0870916465066) (32,0.15661938208261966) (33,0.5892695418909834) (34,2.253226401614621) (35,8.74864814077864)};
    \addplot[dmpcol, solid, mark=*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.7) (3,1.6507936507936507) (4,0.6056344696969697) (5,1.9109844887622665) (6,5.814766029580844) (7,22.014116031027797) (8,7.288019795312536) (9,23.704071982956812) (10,95.31006761700034) (11,377.1256498640919) (12,1475.3709786257914) (13,6513.0329678473845) (14,28575.33074964239) (15,124787.28487222343) (16,27948.697063529187) (17,125836.7654669284) (18,562852.8839121525) (19,2504027.637155473) (20,11090293.581568105) (21,53098618.04878657) (22,253429847.47463083) (23,1206351132.4482615) (24,5729285381.192809) (25,28730718261.215107) (26,143833152334.26038) (27,719010449657.9312) (28,3589690559817.016) (29,18655357447618.79) (30,96855530455119.9) (31,502423927750895.8) (32,66162689529042.875) (33,332901998015967.8) (34,1672767652519972.8) (35,8395146679979751.0)};
    \addplot[dmpcol, solid, mark=square*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.075) (3,0.09523809523809523) (4,0.0032535173160173165) (5,0.004512360067915624) (6,0.00699355514170329) (7,0.014917313079077786) (8,0.0002712533193914343) (9,0.0004493131477970672) (10,0.0009879349229463645) (11,0.002263294818774891) (12,0.005372927219175726) (13,0.014970300123186665) (14,0.04286586583698097) (15,0.12574532538915745) (16,0.0008082588533525322) (17,0.0022776381427943807) (18,0.006547623327042944) (19,0.01916911963095556) (20,0.05706659832528355) (21,0.18719648592607252) (22,0.6228360436215069) (23,2.0996567445800363) (24,7.164869411639471) (25,26.16084879963234) (26,96.53309359385337) (27,359.7327335094123) (28,1352.9754017697553) (29,5348.938431596264) (30,21319.514632747) (31,85627.3631274275) (32,147.96741757700465) (33,551.4673622257629) (34,2070.7428691196474) (35,7831.0708766893995)};
  \end{axis}
\end{tikzpicture}

% ---- sqrtn ----
\begin{tikzpicture}
  \definecolor{smpcol}{rgb}{0.0824,0.3961,0.7529}
  \definecolor{dmpcol}{rgb}{0.7765,0.1569,0.1569}
  \begin{axis}[
    ymode=log,
    xlabel={$n$},
    %ylabel={$\displaystyle\sum_{k\geq k_0}\frac{\|P_k(O)\|_2^2}{\|O\|_\infty^2\, d_k}$},
    title={$p = \lfloor\sqrt{n}\rfloor$},
    legend pos=outer north east,
    legend style={font=\large},
    tick label style={font=\large},
    label style={font=\large},
    title style={font=\large},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    \addplot[smpcol, solid, mark=*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.7) (3,1.6507936507936507) (4,0.9535669191919192) (5,2.4980960372960372) (6,7.724225568670013) (7,26.827811941102972) (8,101.54929809780272) (9,29.422446907282467) (10,104.16023171959797) (11,390.9679167283678) (12,1540.8550315326004) (13,6328.589575899145) (14,26928.848605752093) (15,118153.73876163572) (16,22121.40099611427) (17,91540.80993217549) (18,389053.4355269806) (19,1693538.7089469354) (20,7532670.074926362) (21,34165792.34784907) (22,157747283.66789332) (23,740282063.3614491) (24,3526277312.5205913) (25,469664210.8698487) (26,2138264016.1796043) (27,9874749463.071512) (28,46211365174.41158) (29,218947721935.45386) (30,1049421869167.2264) (31,5084640967742.941) (32,24887579877252.156) (33,122985716518034.9) (34,613248553322498.5) (35,3083959473927130.5)};
    \addlegendentry{$\hat{n}_1^p$, $k_0=0$}
    \addplot[smpcol, solid, mark=square*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.075) (3,0.09523809523809523) (4,0.000615530303030303) (5,0.0008354312354312355) (6,0.0014606792384570162) (7,0.00307224930788642) (9,1.5938077230151574e-05) (10,3.420971654432524e-05) (11,8.078660269041226e-05) (12,0.00020686725430599153) (13,0.0005678229230054961) (14,0.001655357625712395) (15,0.005086997888380507) (16,4.943616865457458e-06) (17,1.368104080635521e-05) (18,3.962228106770109e-05) (19,0.00011956513221986061) (20,0.00037451766451742155) (21,0.001213711514007376) (22,0.0040577573154919975) (23,0.013960046851328506) (24,0.04931150628547201) (25,0.10368210232927909) (26,0.35920978651466223) (27,1.2736726084650356) (28,4.614855505016158) (29,17.062390204854303) (30,64.2911487240527) (31,246.59852817263632) (32,0.15661938208261966) (33,0.5892695418909834) (34,2.253226401614621) (35,8.74864814077864)};
    \addlegendentry{$\hat{n}_1^p$, $k_0=\lfloor\log_2 n\rfloor$}
    \addplot[dmpcol, solid, mark=*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.7) (3,1.6507936507936507) (4,0.6056344696969697) (5,1.9109844887622665) (6,5.814766029580844) (7,22.014116031027797) (8,82.62154629338485) (9,23.704071982956812) (10,95.31006761700034) (11,377.1256498640919) (12,1475.3709786257914) (13,6513.0329678473845) (14,28575.33074964239) (15,124787.28487222343) (16,27948.697063529187) (17,125836.7654669284) (18,562852.8839121525) (19,2504027.637155473) (20,11090293.581568105) (21,53098618.04878657) (22,253429847.47463083) (23,1206351132.4482615) (24,5729285381.192809) (25,1017899947.8981478) (26,4915301854.603311) (27,23663140415.237125) (28,113613841614.43416) (29,544205066917.0765) (30,2601253125906.017) (31,13129865460243.96) (32,66162689529042.875) (33,332901998015967.8) (34,1672767652519972.8) (35,8395146679979751.0)};
    \addlegendentry{$\prod_{i=1}^p \hat{n}_i$, $k_0=0$}
    \addplot[dmpcol, solid, mark=square*, line width=1.5pt, mark size=1.5pt]
      coordinates {(2,0.075) (3,0.09523809523809523) (4,0.0032535173160173165) (5,0.004512360067915624) (6,0.00699355514170329) (7,0.014917313079077786) (9,0.0004493131477970672) (10,0.0009879349229463645) (11,0.002263294818774891) (12,0.005372927219175726) (13,0.014970300123186665) (14,0.04286586583698097) (15,0.12574532538915745) (16,0.0008082588533525322) (17,0.0022776381427943807) (18,0.006547623327042944) (19,0.01916911963095556) (20,0.05706659832528355) (21,0.18719648592607252) (22,0.6228360436215069) (23,2.0996567445800363) (24,7.164869411639471) (25,3.7636476057836634) (26,13.4880862511672) (27,48.71888337088713) (28,177.28463140968788) (29,649.6876327951373) (30,2396.856210734959) (31,9414.704702139228) (32,147.96741757700465) (33,551.4673622257629) (34,2070.7428691196474) (35,7831.0708766893995)};
    \addlegendentry{$\prod_{i=1}^p \hat{n}_i$, $k_0=\lfloor\log_2 n\rfloor$}
  \end{axis}
\end{tikzpicture}


==> plots/Single_Irrep_Observable/Second_Moments.tex <==
% Requires in preamble:
%   \usepackage{pgfplots}
%   \pgfplotsset{compat=1.18}
%   \usepgfplotslibrary{groupplots}
%   \usetikzlibrary{calc}
\begin{tikzpicture}
  \definecolor{maxcol}{rgb}{0.1216,0.4667,0.7059}
  \definecolor{mincol}{rgb}{0.8392,0.1529,0.1569}
  \begin{groupplot}[
    group style={group size=3 by 1, horizontal sep=1.4cm, ylabels at=edge left},
    ymode=log,
    xlabel={$n$},
    ylabel={$\mathbb{E}[f_U^2]$},
    tick label style={font=\footnotesize},
    label style={font=\small},
    title style={font=\small},
    width=0.37\linewidth,
    height=0.32\linewidth,
  ]
    % ===== p = K0 = 2 =====
    \nextgroupplot[title={$p = K_0 = 2$}]
      \addplot[maxcol, solid, mark=o, line width=1.5pt, mark size=1.5pt, forget plot]
        coordinates {(2,0.004761904761904762) (3,0.002976190476190476) (4,0.0011363636363636363) (5,0.0006475006475006475) (6,0.0003391670058336725) (7,0.0002144607843137255) (8,0.00013168644650842794) (9,9.022556390977444e-05) (10,6.098249576510446e-05) (11,4.4283413848631237e-05) (12,3.1919383771235626e-05) (13,2.420234651058015e-05) (14,1.8268868011212114e-05) (15,1.4319098240469209e-05) (16,1.119055576776165e-05) (17,9.003712707416411e-06) (18,7.2297018365894255e-06) (19,5.941213258286429e-06) (20,4.8753477567998275e-06) (21,4.076902020396158e-06) (22,3.405589754317975e-06) (23,2.889749280326788e-06) (24,2.450054095712359e-06) (25,2.104911837030653e-06) (26,1.8072475368445002e-06) (27,1.569322192308229e-06) (28,1.3620359179297019e-06) (29,1.1937472343140584e-06) (30,1.0458277101440625e-06) (31,9.240976037851038e-07) (32,8.162653189472219e-07)};
      \addplot[mincol, solid, mark=o, line width=1.5pt, mark size=1.5pt, forget plot]
        coordinates {(2,0.00873015873015873) (3,0.0011243386243386243) (4,0.00016233766233766234) (5,4.604449048893493e-05) (6,1.4046310342606638e-05) (7,5.7234432234432234e-06) (8,2.4299284772388486e-06) (9,1.2121807787442463e-06) (10,6.205236411186068e-07) (11,3.5203658392064187e-07) (12,2.0326353301840866e-07) (13,1.2602405283615699e-07) (14,7.913429076314334e-08) (15,5.235444786334664e-08) (16,3.497048677425516e-08) (17,2.4310118718252343e-08) (18,1.702606408243386e-08) (19,1.2306174052002036e-08) (20,8.94800667914678e-09) (21,6.674204955684215e-09) (22,5.002582352379442e-09) (23,3.82938267466115e-09) (24,2.943263155888395e-09) (25,2.3025158054049594e-09) (26,1.8074572186564092e-09) (27,1.440344211017525e-09) (28,1.151174451352665e-09) (29,9.320619485404454e-10) (30,7.565764459383633e-10) (31,6.210990189374642e-10) (32,5.110147946078158e-10)};
    % ===== p = log2(n) =====
    \nextgroupplot[title={$p = \log_2(n)$}]
      \addplot[maxcol, solid, mark=o, line width=1.5pt, mark size=1.5pt, forget plot]
        coordinates {(2,0.05) (4,0.0011363636363636363) (8,8.918447170941152e-06) (16,1.1736051880933848e-08) (32,2.312045796653745e-12) (64,4.259094826846709e-17) (128,6.62413340961674e-23)};
      \addplot[mincol, solid, mark=o, line width=1.5pt, mark size=1.5pt, forget plot]
        coordinates {(2,0.016666666666666666) (4,0.00016233766233766234) (8,1.021124728605657e-07) (16,2.2289014549417563e-12) (32,1.692513628455208e-18) (64,3.147435242102916e-26) (128,1.4145254691724165e-35)};
    % ===== p = sqrt(n) =====
    \nextgroupplot[title={$p = \lfloor\sqrt{n}\rfloor$}]
      \addplot[maxcol, solid, mark=o, line width=1.5pt, mark size=1.5pt, forget plot]
        coordinates {(4,0.0011363636363636363) (9,4.794105989122516e-06) (16,1.1736051880933848e-08) (25,1.825674500271331e-11) (36,1.947573434665783e-14) (49,1.5079345998485534e-17) (64,8.844090281100399e-21) (81,4.0611754128113315e-24) (100,1.4988132111120314e-27) (121,4.540997787636844e-31)};
      \addplot[mincol, solid, mark=o, line width=1.5pt, mark size=1.5pt, forget plot]
        coordinates {(4,0.00016233766233766234) (9,3.215860570618819e-08) (16,2.2289014549417563e-12) (25,6.956635928579644e-17) (36,1.1488679490822735e-21) (49,1.1192223640088939e-26) (64,6.951436986145973e-32) (81,2.9172064045052434e-37) (100,8.652201427594675e-43) (121,1.8797811584923854e-48)};
  \end{groupplot}

  % ===== Full-width legend rectangle below the row (two entries) =====
  \coordinate (L) at (group c1r1.south west);
  \coordinate (R) at (group c3r1.south east);
  \begin{scope}[every node/.style={anchor=west, font=\small, inner sep=0pt}]
    \def\lw{0.6cm}      % line-sample width
    \def\gap{0.18cm}    % gap sample->text
    \def\drop{1.45cm}   % distance below plots to legend row
    \coordinate (e1) at ($(L)!0.22!(R) - (0,\drop)$);
    \coordinate (e2) at ($(L)!0.55!(R) - (0,\drop)$);
    % Max bunching (blue)
    \draw[maxcol, solid, line width=1.5pt] (e1) -- ++(\lw,0);
    \node[draw=maxcol, circle, inner sep=1.7pt, line width=1pt] at ($(e1)+(0.5*\lw,0)$) {};
    \node at ($(e1)+(\lw+\gap,0)$) {Max Bunching};
    % Min bunching (red)
    \draw[mincol, solid, line width=1.5pt] (e2) -- ++(\lw,0);
    \node[draw=mincol, circle, inner sep=1.7pt, line width=1pt] at ($(e2)+(0.5*\lw,0)$) {};
    \node at ($(e2)+(\lw+\gap,0)$) {Min Bunching};
    % full-width box
    \draw[black] ($(L)+(0,-\drop+0.4cm)$) rectangle ($(R |- e1)+(0,-0.4cm)$);
  \end{scope}
\end{tikzpicture}

==> plots/Single_Irrep_Observable/Single_Irrep_Purities.tex <==
% sec1_purity_evolution — generated by Single_Irrep_Observable.ipynb
% Requires: \usepackage{pgfplots} \pgfplotsset{compat=1.18}
\begin{tikzpicture}
  \begin{axis}[
    xmode=log, ymode=log,
    xlabel={$n$},
    legend pos=north west,
    legend style={
      draw=black,
      fill=white,
      font=\small,
    },
    tick label style={font=\normalsize},
    label style={font=\normalsize},
    title style={font=\normalsize},
    width=0.85\linewidth,
    height=0.65\linewidth,
  ]
    \addplot[cyan, only marks, mark=*, mark size=3pt]
      coordinates {(2,3.0) (4,19.5) (8,8222.5) (16,9922086868.75) (32,5.991728752438885e+22) (64,6.91841904300876e+48) (128,2.675631769238699e+101)};
    \addlegendentry{$\mathrm{Tr}[O O^\dagger]$}
    \addplot[orange, only marks, mark=square*, mark size=3pt]
      coordinates {(2,2.0) (4,4.0) (8,40.5) (16,4096.0) (32,3500658.0) (64,33493575156.25) (128,3635209839381768.0)};
    \addlegendentry{$\|O\|_\infty^2$}
  \end{axis}
\end{tikzpicture}
